Quality with Just Enough Diversity in Evolutionary Policy Search

Evolution Strategies (ES) are effective gradient-free optimization methods that can be competitive with gradient-based approaches for policy search. ES only rely on the total episodic scores of solutions in their population, from which they estimate fitness gradients for their update with no access to true gradient information. However this makes them sensitive to deceptive fitness landscapes, and they tend to only explore one way to solve a problem. Quality-Diversity methods such as MAP-Elites introduced additional information with behavior descriptors (BD) to return a population of diverse solutions, which helps exploration but leads to a large part of the evaluation budget not being focused on finding the best performing solution. Here we show that behavior information can also be leveraged to find the best policy by identifying promising search areas which can then be efficiently explored with ES. We introduce the framework of Quality with Just Enough Diversity (JEDi) which learns the relationship between behavior and fitness to focus evaluations on solutions that matter. When trying to reach higher fitness values, JEDi outperforms both QD and ES methods on hard exploration tasks like mazes and on complex control problems with large policies.

==> jedi.tex <==
\chapter{Behavior information in Neural Policy Search}
\minitoc

\textit{\textbf{Note:} This work has been submitted for review at GECCO 2024.}

\section{Motivation}

Methods such as \mapelites{} present the goal of Quality-Diversity optimization as twofold:
\begin{itemize}
  \item Create a population of policies with diverse behaviors and high fitness values
  \item Use different behaviors as stepping stones
\end{itemize}

However while QD methods can reach high fitness values when taking the best performing individual, a large portion of the evaluation budget is used to improve non-best individuals in order to have a globally well-performing archive.

On the other hand, Evolution Strategies focus purely on reaching the highest possible fitness on one individual, with no information from the behavior of policies. In a way, this approach could hence be called "Quality-Quality" (QQ) optimization. Since these methods do not keep a diversity of policies, they cannot benefit from the stepping stones of QD.

In this work we try to bridge the gap between QD and QQ by introducing the \textit{\longjedi} (or \jedi{}) framework. The aim of \jedi{} is to explore the behavior space enough to gain an idea of which behaviors might perform well while still focusing only on reaching the highest possible max fitness like an ES.



\subsection{Archive comparison}
In order to highlight differences between QD and QQ methods, we compare the behavior space coverage and evaluation budget dispersion of \mapelites{} and \sepcmaes{} on the \pointmaze{} environment. We run them for the same evaluation budget, and log all the evaluated samples of \sepcmaes{} in an archive similar to \mapelites{}.

The goal of \pointmaze{} is to reach a target position in the top left corner of a maze, starting from the bottom right corner. The reward at each timestep is the distance to the goal, and the episode ends when the agent reaches the goal or after 100 steps. The final fitness is the sum of rewards over the episode.

\subsubsection{Coverage}

\begin{figure}[h]
  \begingroup
  \centering
  \subfloat[\mapelites{} coverage]{{\includegraphics[width=0.45\textwidth]{images/JEDi/me_coverage.png} }}%
  \qquad
  \subfloat[ES coverage]{{\includegraphics[width=0.45\textwidth]{images/JEDi/es_coverage.png} }}%
  \endgroup
  \caption{Coverage of \mapelites{} and ES on \pointmaze{}}
  \label{fig:coverage}
\end{figure}

We show coverage maps in \Cref{fig:coverage}. The coverage of \mapelites{} is much higher than the coverage of ES, which is expected since \mapelites{} explicitly tries to cover the behavior space while ES does not. ES gets stuck in local optima of the higher wall, where reaching the goal requires to go further away from it first. \mapelites{} gets closer, and with more budget would reach it, by covering the behavior space leading to it.

\pt{Explain difference diversity / coverage: 50\% coverage is not the same if it's dense or not}

\subsection{Evaluation budget}

\begin{figure}[h]
  \begingroup
  \centering
  \subfloat[\mapelites{} budget dispersion]{{\includegraphics[width=0.45\textwidth]{images/JEDi/me_count.png} }}%
  \qquad
  \subfloat[ES budget dispersion]{{\includegraphics[width=0.45\textwidth]{images/JEDi/es_count.png} }}%
  \endgroup
  \caption{Budget dispersion of \mapelites{} and ES}
  \label{fig:count}
\end{figure}

In \Cref{fig:count} we show the number of evaluations made in each cell of the behavior archive. We can see that \mapelites{} has a more homogeneous distribution of evaluations, covering much of the behavior space. On the other hand, ES has a very heterogeneous distribution of evaluations, with some cells in the local optimum having a lot of evaluations and many others having none. This shows ES focuses its evaluation budget on what it believes to be the best behavior, while \mapelites{} tries to cover the whole behavior space.

In a deceptive problem the ES gets stuck in a local optimum while the extensive exploration of \mapelites{} allows to find the solution, but in other problems the ES focusing its budget on the best behavior can be beneficial by reaching higher fitness values faster. Meanwhile \mapelites{} spends a lot of budget on finding the best policy for each behavior, even if that behavior will not lead to high fitness values, and hence can be slower to reach high fitness values.

In order to find a balance between them we introduce \longjedi{} (\jedi{}), which uses an archive to estimate the relationship between behavior and fitness and uses it to select target behaviors to reach with an ES. This allows \jedi{} to focus on reaching high fitness values while still exploring the behavior space enough to find good behaviors.

Concretely, we want \jedi{} to converge to high fitness values faster than QD methods and not get stuck like ES on hard exploration problems.

\section{Quality with Just Enough Diversity}

\subsection{Main loop}

\subsubsection{\jedi}
The first step is to sample a population of random agents, evaluate them and add them to the archive. The main loop of \jedi{} then relies on 4 steps:
\begin{enumerate}
  \item Estimate the relationship between behavior and fitness with a gaussian process based on the archive
  \item Select promising target behaviors
  \item Run an ES to reach each behavior and maximize fitness
  \item Update the archive with the agents sampled by the ES
\end{enumerate}

The whole pseudocode for \jedi{} is presented in \Cref{algo:jedi} and shown in \Cref{fig:jedi_loop}.

\begin{algorithm}[h]
  \caption{\jedi}
  \label{algo:jedi}
  \begin{algorithmic}
    \STATE $\mathcal{S}$ - \jedi{} scoring function
    \STATE $\mathcal{T}$ - \jedi{} target selection function
    \STATE $n_{ES}$ - Number of ES emitters
    \STATE $L$ - Number of \jedi{} loops


    \STATE $\mathcal{R}$ - Repertoire
    \STATE $r$ - Rollout function

    \STATE $N$ - Number of ES loops
    \STATE $\lambda$ - ES population size
    \STATE $\theta$ - ES parameters
    \STATE $\mathcal{U}$ - ES update function


    \FOR{$l \in \{1, ..., L\}$}
    \STATE Sample $n_{ES}$ behavior targets: $(t_i)_{1..n_{ES}} = \mathcal{T}(\mathcal{R}, n_{ES})$

    \FOR{$i \in \{1, ..., n_{ES}\}$}
    \STATE Select the starting genome from the repertoire: $\phi_0, d_0 = \argmin_{\phi, d \in \mathcal{R}} \| d - t_i \|$
    \STATE Initialize the ES parameters: $\theta_{\phi_0} = \phi_0$
    \FOR{$j \in \{1, ..., N\}$}
    \STATE Sample $\lambda$ genomes from the ES parameters: $\{\phi_k\}_{k \in \{1, ..., \lambda\}} \sim \theta$
    \STATE Get fitness values and descriptors: $\forall k, (f_k, d_k) = r(\phi_k)$
    \STATE Compute scores: $\forall k, s_k = \mathcal{S}(f_k, d_k, t_i)$
    \STATE Update $\theta$ using scores: $\theta = \mathcal{U}(\theta, (\phi_k)_k, (s_k)_k)$
    \ENDFOR
    \ENDFOR

    \STATE Update the repertoire $\mathcal{R}$ with all evaluated genomes.
    \ENDFOR
  \end{algorithmic}
\end{algorithm}

\begin{figure}[h]
  \centering
  \includegraphics[width=\textwidth]{images/JEDi/jedi_loop.png}
  \captionof{figure}{\jedi{} main loop on a \pointmaze{} example.}
  \label{fig:jedi_loop}
\end{figure}

\subsubsection{Differences with ES}
\jedi{} actively uses behavior information which is usually not available to standard ES methods. This allows to explore the behavior space to inform the search in genome space.

\subsubsection{Differences with \mapelites{}}
In \mapelites{} the exploration happens via random mutations on agents from the archive, hoping offsprings will reach new behaviors. Selection pressure is applied through the archive, where new solutions are only kept if they are better than the current best in their behavior cell or if they reach a new behavior. In \jedi{} the exploration happens via the target choice, actively targeting behaviors that can be useful to reach higher fitness values.

\subsubsection{Differences with CMA-ME and ME-ES}
\jedi{}, CMA-ME and ME-ES all use ES in a \mapelites{} archive. However, CMA-ME and ME-ES use ES to improve the overall archive based on fitness alone instead of targeting behaviors to explore the behavior space. The CMA-ME-rnd variant of CMA-ME uses random behavior directions to explore the behavior space, but does not maximize fitness at the same time and the direction is random instead of being based on the behavior-fitness relationship.


\subsection{Gaussian Process}
\pt{Manuscript: Motivate why we use GP, what it is, how it is trained}

In order to learn a global relationship between behavior and fitness we approximate the landscape with a Gaussian Process (GP) which is fit on a \mapelites{} Archive.

\subsubsection{Gaussian Process}

In a \mapelites{} repertoire, each point kept is the best performing genome in its behavior cell, hence the relationship that can be learnt is the link between a behavior and the fitness of the best individual found so far that showcased that behavior.

\begin{equation}
  \mu(x) = k(x, X) (K + \sigma_n^2 I)^{-1} y
\end{equation}

\begin{equation}
  \sigma^2(x) = k(x, x) - k(x, X) (K + \sigma_n^2 I)^{-1} k(X, x)
\end{equation}

with $x$ the behavior for which to predict the fitness, $X$ the behaviors in the archive which have a solution, $y$ their respective fitness values, $\sigma_n$ the observation noise, $k$ the GP kernel and $K$ the kernel matrix so that $\forall i, j$ with $x_i$ and $x_j$ behaviors of the repertoire:

\begin{equation}
  K_{ij} = k(x_i, x_j)
\end{equation}


\subsubsection{Weighted Gaussian Process}

In a \mapelites{} repertoire, the value of each cell is actually the result of multiple evaluations where the highest fitness is kept. If we count each cell as 1 point in the GP, a full archive will be considered as a homogeneously explored space no matter how many evaluations were made in each cell and hence the uncertainty landscape will be flat. In order to consider the distribution of evaluation budget over the behavior space, we use a weighted Gaussian Process \citep{calandrielloScalingGaussianProcess2022}.

Given the evaluation budget $n_i$ of a cell with behavior $x_i$, its weight in the diagonal weight matrix $W$ is defined as:

\begin{equation}
  W_{ii} = \frac{1}{n_i}
\end{equation}

and then used in the GP prediction for the fitness of a behavior $x$:

\begin{equation}
  \mu(x) = k(x, X) (K + \sigma_n^2 W)^{-1} y
\end{equation}

\begin{equation}
  \sigma^2(x) = k(x, x) - k(x, X) (K + \sigma_n^2 W)^{-1} k(X, x)
\end{equation}



\subsection{Target behavior selection}
\pt{Manuscript: More details, be more explicit}

Once the GP is trained on the archive, it can be used to predict the fitness and standard deviation of the fitness of any behavior. We compute them for each centroid of the archive and consider the selection of targets as a trade-off between exploration (behaviors with high standard deviation) and exploitation (behaviors with high predicted fitness).

\subsubsection{GP-UCB}
In order to select the next target behavior we can use the GP-UCB (Gaussian Process Upper Confidence Bound, \citet{srinivasGaussianProcessOptimization2012}) acquisition function, which uses the Upper Confidence Bound (UCB) method to select the next target behavior. The UCB is defined as:

\begin{equation}
  UCB(x) = \mu(x) + \sqrt{\beta} \sigma(x)
\end{equation}

with $\mu(x)$ the mean of the GP at $x$, $\sigma(x)$ the standard deviation of the GP at $x$ and $\beta$ a parameter that controls the exploration-exploitation trade-off. The higher $\beta$ is, the more the algorithm will explore.

Since the GP mean and std are continuous, using GP-UCB to select a batch of multiple targets to parallelize ES will result in many targets around the same area. In order to improve the diversity of the targets, the GP-BUBC (Gaussian Process Batch Upper Confidence Bound, \citet{desautelsParallelizingExplorationExploitationTradeoffs}) method updates the GP standard deviation (which only depends on where the evaluation was made and not its result) after sampling each target of the batch, effectively hallucinating the evaluation of the other targets of the batch. This results in a more diverse batch of targets.

\subsubsection{Pareto front}
In order to simplify the batch sampling approach and select multiple target behaviors that are both promising and uncertain, we instead consider it as a multi-objectif optimization problem where we try to maximize both the GP mean and standard deviation. Considering the Pareto front of the GP predictions allows to select multiple targets that are both promising and uncertain as seen in \Cref{fig:pareto}. This allows to select a batch of targets that are more diverse than with GP-UCB without hallucinating evaluations.

We first evaluate the GP for each centroid in the repertoire, discretizing the behavior space, to get the mean and standard deviation of the GP at each point. We then compute the Pareto front of the GP predictions and from these points we randomly select $n_{ES}$ target behaviors to reach with an ES each.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\textwidth]{images/JEDi/pareto.png}
  \captionof{figure}{Pareto front of the GP predictions}
  \label{fig:pareto}
\end{figure}




\subsection{Weighted scoring function}




Once a target behavior $d_{target}$ has been picked, we want to solve the problem of maximizing the fitness $f$ under the constraint of staying close to the target behavior:

\begin{equation} \label{eq:jedi_problem}
  \max_{\phi} f(\phi) \quad \text{ s.t. } \quad \| d(\phi) - d_{target} \| \leq \epsilon
\end{equation}

Previous works such as ARIA \citep{grillottiDonBetLuck2023} have tackled the use of ES to reach behavior descriptors and maximize the fitness at the same time. The ARIA ES scoring function ranks first solutions that reached the target cell, ranked between themselves based on fitness, and then the others based on how close they are to the target behavior (\Cref{eq:aria}). This allows to use extra budget to improve fitness once the target is reached.

\begin{equation}\label{eq:aria}
  \mathcal{S}_{ARIA}(x_i) = \begin{cases}
    f(x_i)                               & \text{if } \| d(x_i) - d_{target} \| \leq \epsilon \\
    f_{min} -  \| d(x_i) - d_{target} \| & \text{otherwise}
  \end{cases}
\end{equation}
with $f_{min}$ the minimum fitness value in the current ES population and $\epsilon$ the maximum distance to the target behavior.

However, this scoring function does not allow to pick a balance between exploration and exploitation and it depends on the choice of $\epsilon$. In order to do so, we use the Lagrangian relaxation of the problem and we introduce the\longwtf{} (\wtf{}) as a way to combine the goal of reaching a target and the fitness reached in the environment. The WTFS is defined in \Cref{eq:wtf}:

\begin{equation}\label{eq:wtf}
  \mathcal{S}_{\wtf{}}^\alpha(x_i) = \alpha \mathcal{S}_{target}(x_i) + (1 - \alpha) \mathcal{S}_{fitness}(x_i)
\end{equation}

with $\alpha$ the weight of the target behavior in the scoring function. $\alpha = 0$ corresponds to pure exploitation, $\alpha = 1$ to pure exploration and $\alpha = 0.5$ to a balance between the two. Having a scalar control the balance between exploration and exploitation allows to use a linear schedule to first focus on exploration and then on exploitation.

We normalize the target and fitness scores to be between 0 and 1, both being maximized. For fitness values, with $f_{min}$ and $f_{max}$ the minimum and maximum fitness values in the current ES population, we have:

\begin{equation}
  \mathcal{S}_{fitness}(x_i) = \frac{f(x_i) - f_{min}}{f_{max} - f_{min}}
\end{equation}

To reach a target behavior, we minimize the Euclidian distance between the behavior descriptor $d(x_i)$ of an individual $x_i$ and the target behavior descriptor $d_{target}$:

\begin{equation}
  \mathcal{S}_{target}(x_i) = 1 - \frac{\| d(x_i) - d_{target} \| - d_{min}}{d_{max} - d_{min}}
\end{equation}

with $d_{min}$ and $d_{max}$ the minimum and maximum distance between the target behavior and behavior descriptors of the current ES population.

To set the value of $\alpha$, we either set it to a fixed value or we use a linear schedule that starts at 1 and ends at 0, updated at each loop of \jedi{} and fixed for each ES rollout. This allows \jedi{} to first focus on exploration through reaching target behaviors, and later on to focus on exploitation through reaching high fitness values.


\subsection{Results}



\subsubsection{Baselines}

In this work we focus on tasks where we consider neither fitness nor behavior to be differentiable, hence not comparing directly to methods that use RL such as PGA-ME \citep{nilssonPolicyGradientAssisted2021a} or Differentiable QD such as QD-RL \citep{cideronQDRLEfficientMixing2020}. We hence use 3 types of baselines:
\begin{itemize}
  \item Evolution Strategies, specifically \sepcmaes{}
  \item ES-free Quality-Diversity methods, specifically \mapelites{}
  \item QD + ES methods, specifically CMA-ME and CMA-MAE
\end{itemize}

Extensions of \jedi{} to include RL or differentiable QD components are left for future work.

\subsubsection{Exploration problem}
\pt{PointMaze}

\subsubsection{Hard exploration and robot control}
\subsubsubsection{Custom trap position}
\pt{AntTrap custom trap position}

\subsubsubsection{Maze with robotic control}
\pt{AntMaze}


\subsubsection{Decorrelating BD from fitness}
\pt{HalfCheetah}

\subsubsection{Handling stochasticity}
\pt{Random seed for each eval = noise in fitness and in bd}



\subsection{Conclusions}
\subsubsection{Convergence speed}

\pt{JEDi converges faster than QD baselines, and doesn't get stuck on hard exploration problems like ES}

\subsubsection{Bad coverage by design}
\pt{Worse QD score for JEDi because we explicitly try not to cover the whole BD space, so the QD score is not a good metric for JEDi performance.}

\subsubsection{Future work}

